Sub-Riemannian interpolation inequalities

We prove that ideal sub-Riemannian manifolds (i.e., admitting no non-trivial abnormal minimizers) support interpolation inequalities for optimal transport. A key role is played by sub-Riemannian Jacobi fields and distortion coefficients, whose properties are remarkably different with respect to the Riemannian case. As a byproduct, we characterize the cut locus as the set of points where the squared sub-Riemannian distance fails to be semiconvex, answering to a question raised by Figalli and Rifford in [Geom. Funct. Anal. (2010) 20: 124]. As an application, we deduce sharp and intrinsic Borell-Brascamp-Lieb and geodesic Brunn-Minkowski inequalities in the aforementioned setting. For the case of the Heisenberg group, we recover in an intrinsic way the results recently obtained by Balogh, Krist\'aly and Sipos in [Calc. Var. PDE (2018) 57: 61], and we extend them to the class of generalized H-type Carnot groups. Our results do not require the distribution to have constant rank, yielding for the particular case of the Grushin plane a sharp measure contraction property and a sharp Brunn-Minkowski inequality.

==> superdiff.tex <==
\section{Super-differentiability of distance}\label{a:superdiff}
{\blue 
The result of Lemma~\ref{l:superdiff} is slightly stronger than super-differentiability of the squared sub-Riemannian distance at point reached by at least one normal minimizing geodesic. The super-differentiability of the squared distance in the Riemannian case  is proved, for example, in \cite{McCann-polar}. Notice that here we do not use geodesic equations or normal neighborhoods as in the latter reference, since they are not available in the sub-Riemannian setting.
\begin{lemma}\label{l:superdiff}
Let $x \neq y \in M$, and let $z\mapsto f(z):= d^2_{SR}(z,y)/2$.  Assume that there exists a normal minimizing geodesic joining $y$ with $x$. Then there exists coordinates around $x$, and $p \in \R^n$ such that
\begin{equation}
f(x+v) - f(x) \leq p \cdot v + O(|v|^2), \qquad \forall |v| < 1.
\end{equation}
\end{lemma}
\begin{proof}
Let $u \in L^2([0,1],\R^m)$ be the control associated with a normal minimizing geodesic $\gamma_u$ joining $y$ with $x$, that is such that that $E_y(u) = x$. 


We first observe that there exists an $n$-dimensional subspace $\mathcal{V} \subset L^2([0,1],\R^m)$ of controls such that
\begin{equation}
A : \mathcal{V} \to M, \qquad A(\delta u) := E_y(u+\delta u),
\end{equation}
is a $C^1$-diffeomorphism between a neighborhood of $0 \in \mathcal{V}$ and a neighborhood of $x =A(0) \in M$. \todo{Dico $C^1$ perche' Riff dice solo $C^1$ ma penso sia smooth.} This property is a standard ingredient in the proof of the openness of the endpoint map, see \cite[Proposition 1.4.1]{riffordbook}\todo{Mettere il numero giusto della versione stampata che non ho qui.} or \cite[Lemma 3.32]{nostrolibro}.

Taking this property for granted, we proceed with the proof of the lemma. Without loss of generality, we assume that $M = \R^n$, and that $A$ is a diffeomorphism between $\mathcal{V}' \subset \mathcal{V}$ and the unit ball $B_1(x)\subset M$ centered at $x$. For any fixed $|v| <1$, let $\delta u \in \mathcal{V}'$ such that $A(\delta u) = x+v$. Then, we have
\begin{align*}
f(x+v)-f(x) & \leq J(u+\delta u) - J(u) & & \text{by minimality of $\gamma_u$} \\
& = (D_u J) (\delta u) + O(\| \delta u \|^2_2) & & \text{by smoothness of $J$}\\
& = p \cdot d_u E_y (\delta u) + O(\| \delta u \|^2_{2}) & &  \text{by Lagrange multipliers} \\
& = p\cdot \left(E_y(u+\delta u)-E_y(u)\right)+ O(\| \delta u \|^2_{2}) & & \text{by smoothness of $E_y$} \\
& =p\cdot v + O(|v|^2).
\end{align*}
In the last line we used the fact that $A: \mathcal{V}' \to B_1(x)$ is a $C^1$-diffeomorphism, hence there exists $c>0$ such that for all $|v|<1$ and $\delta u = A^{-1}(x+v)$, it holds
\begin{equation}
c^{-1} |v| \leq \|\delta u\|_{2} \leq c |v|, \qquad \forall\, |v| <1. \qedhere
\end{equation}
\end{proof}
}
